Data-driven control of infinite dimensional systems: Application to a continuous crystallizer

Controlling infinite dimensional models remains a challenging task for many practitioners since they are not suitable for traditional control design techniques or will result in a high-order controller too complex for implementation. Therefore, the model or the controller need to be reduced to an acceptable dimension, which is time-consuming, requires some expertise and may introduce numerical error. This paper tackles the control of such a system, namely a continuous crystallizer, and compares two different data-driven strategies: the first one is a structured robust technique while the other one, called L-DDC, is based on the Loewner interpolatory framework.

==> EDF.tex <==

\section{Application to an hydroelectricity generation channel}
\label{appli_EDF}
The second application is an industrial problem provided by the French power producer EDF (Electricit\'e de France). EDF uses water resources to generate green energy with run-of-the-river power plants. They rely on open-channel hydraulic systems that are non-linear and which dynamic depends on the operating point. Here, for simplicity we will consider one single operating point only.
\par  \leavevmode \par 
Their physical model requires partial differential equations (namely Saint-Venant equations). In \cite{EDF}, a new irrational transfer function is proposed for open channels to represent the level-to-flow variations for any operating point. It is the solution of Saint-Venant equations under many assumptions. The system has two inputs, the entering and the outgoing flows $q_e$ and $q_s$, and one output, the water depth $h$. The transfer is given by: 
\begin{equation}
\begin{array}{ccl}
h(x,s,Q_0) & =  & G_e(x,s,Q_0)q_e(s)+G_s(x,s,Q_0)q_s(s) \\
 & = & P(x,s,Q_0)\left[ \begin{array}{c} q_e \\ q_s \end{array}\right]
 \end{array},
 \label{EDF_eq}
\end{equation}
where
$$\begin{array}{r@{=}l}
G_e(x,s,Q_0) &   \frac{\lambda_1(s)e^{\lambda_2(s)L+\lambda_1(s)x}-\lambda_2(s)e^{\lambda_1(s)L+\lambda_2(s)x}}{B_0s(e^{\lambda_1(s)L}-e^{\lambda_2(s)L})}\\
G_s(x,s,Q_0) &  \frac{\lambda_1(s)e^{\lambda_1(s)x}-\lambda_2(s)e^{\lambda_2(s)x}}{B_0s(e^{\lambda_1(s)L}-e^{\lambda_2(s)L})}
\end{array}$$
where $x$ is the position of the measurement point on the channel, $Q_0$ the nominal flow, $L$ the length of the open channel. $B_0$, $\lambda_1(s)$ and $\lambda_2(s)$ depend on the canal configuration and the nominal flow (see \cite{EDF}). 
\par \leavevmode \par 
The system, which dynamic is visible in Figure \ref{transfertEDF_parametrique}, is extremely slow, has a delay behavior and a pole in limit of stability. Moreover, it has an infinite number of poles since the transfer function is irrational. 
\begin{figure}
    \centering
    \includegraphics[scale=0.4]{EDF/plant_model.pdf}
    \caption{System dynamic for nominal flow $Q_0=1400\ m^3.s^{-1}$: original plant in solid blue and approximation obtained in \cite{EDF} in dashed red.}
    \label{transfertEDF_parametrique}
\end{figure}
\par \leavevmode \par 
The system have been approximated in \cite{EDF} by a 8th order rational transfer function depending on the nominal flow with input time delays: $\tau_e\simeq500s$ and $\tau_s\simeq1500s$, on $q_e$ and $q_s$ respectively. This approximation is shown in Figure \ref{transfertEDF_parametrique} (dashed red). This model will be used to evaluate the performances of the identified controller.
\par \leavevmode \par 
The input flow $q_e$ in the open channel is seen as a disturbance (rain for example). The objective is to maintain the water depth to avoid flooding in the area. To this aim, the command signal is the output flow $q_s$. Therefore, only the transfer $G_s$ between the output flow $q_s$ and the water depth $h$ is considered, see \eqref{EDF_eq}.
\par \leavevmode \par 
In this example, the frequency approach is interesting since the system is represented by an irrational transfer function. Therefore, one cannot have a time-domain simulation. However we still can estimate samples of the frequency response of the system $\{\omega_{i},\Phi_{i}\}, \ i=1 \ldots N$, from which the ideal controller's frequency response can be deduced. The samples of the frequency response $\Phi_{i}=G_s(\imath\omega_{i}), \ i=1 \ldots N$ are extracted from the irrational transfer function $G_s$, for $N=500$ linearly spaced frequencies between $10^{-4}$ and $10^{-1}$ rad.s$^{-1}$.
\par\leavevmode\par
As for the previous application, the first step of the proposed method consist in determining the nature of the system thanks to the projection of its frequency-response measurements. The results of steps 1 and 2 of Algorithm \ref{algo_choixM} are visible on Figures \ref{proj_EDF} and \ref{inv_proj_EDF} respectively. 
\par \leavevmode \par 
Due to the presence of an integrator, the data of the plant is filtered by a bandpass filter for the stability analysis, see \cite{cooman2018model} for further explanations. Figure \ref{proj_EDF} shows that, except the integrator, the plant has no unstable poles. The mismatch between the projection and the plant's data is due to the use of the bandpass filter. According to Figure \ref{inv_proj_EDF}, the plant is minimum phase: the stable projection fits the inverse of the plant's data.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/plant_projection.pdf}
    \caption{Projection of the plant's data: the only instability is the integrator.}
    \label{proj_EDF}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/inv_projection.pdf}
    \caption{Projection of the inverse of the plant's data: the system is minimum phase.}
    \label{inv_proj_EDF}
\end{figure}
\par \leavevmode \par 
Therefore, the only constraint that the reference model should satisfy is $M(0)=1$, which would have been respected anyway to have zero tracking error. The objective is to stabilize the system and to obtain a faster dynamic. The reference closed-loop $M$ is chosen to be a second order continuous transfer function:
\begin{equation}
    M(s)=\frac{1}{1+\frac{2\xi}{\omega_0}s+\frac{s^2}{\omega_0^2}},
    \label{M_EDF}
\end{equation}
with $\omega_0=10^{-4} rad.s^{-1}$ and $\xi=1$. It satisfies $M(0)=1$.

\par \leavevmode \par 
The frequency response of the ideal controller $K(\imath\omega_{i})$, which exactly provides the desired closed-loop behavior dictated by $M$ when placed in the closed-loop, is obtained as follows:
$$\forall i=1\ldots N, \ K(\imath\omega_{i})=\frac{M(\imath\omega_{i})}{\Phi_{i}-M(\imath\omega_{i})\Phi_{i}} .$$

\par \leavevmode \par
The result of the identification step is given in Figure \ref{id_K_EDF}. The minimal realisation of the ideal controller is of order 137 and is stable. It is then reduced to a stable second order controller:
$$K(s)=\frac{3.3492e-05 (s^2 - 0.0663s + 0.007729)}{(s+2.001e-05) (s+0.001161)}.$$

\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/idK_EDF.pdf}\\
    \caption{Identification of the ideal controller (red dots): minimal realization of order 137 (solid blue) and reduced 2nd order LDDC controller(dashed blue).}
    \label{id_K_EDF}
\end{figure}
\par \leavevmode \par 
Since we had no access to the EDF simulator, the 8th order rational transfer function of \cite{EDF} is used to simulate the closed-loop with the 2nd order controller obtained by the LDDC. The results are shown in Figure \ref{simul_temp_EDF_1}: the resulting closed-loop achieve a response time of $4.84\times10^5$s (134.4 hours) with no overshoot, while the system naturally has a response time of $2.47\times10^{13}$s. The closed-loop dynamic is almost the objective one. The command signal is shown on Figure \ref{simul_temp_EDF_u}: it is reasonable, the maximum flow variation is around $8.3m^3.s^{-1}$, which is in the acceptable range for this application with a controller of order 2.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/step_EDF.pdf}
    \caption{Step response of the closed loop using the 2nd order LDDC controller (dashed green) and of the objective transfer (solid red).}
    \label{simul_temp_EDF_1}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/step_command_EDF.pdf}
    \caption{Evolution of the outgoing flow $q_s$ when applying a step on the closed-loop obtained with the identified 2nd order controller $K$.}
    \label{simul_temp_EDF_u}
\end{figure}

\par \leavevmode \par 
Finally, the performances in terms of disturbance rejection are shown on Figure \ref{EDF_dist}: an input flow of $100m^3/s$ during four hours is considered. This disturbance would increase the water depth of $0.65m$ if not rejected. Figure \ref{EDF_dist} represents the tracking error when this disturbance is applied on the stabilized closed-loop: the water depth increases of $0.54m$ instead of the $0.65m$ without the controller. Finally, the disturbance is completely rejected $0.8\times 10^{5}s$ (2.3 hours) after its application. During the remaining time of the disturbance application, the disturbance does not affect the closed-loop system.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.75\textwidth]{EDF/dist_EDF.pdf}
    \caption{Performance of the controlled closed-loop in terms of disturbance rejection.}
    \label{EDF_dist}
\end{figure}

\par \leavevmode \par
It should be noted that the closed-loop could be faster by increasing the frequency $\omega_0$ of the reference model $M$, see \eqref{M_EDF}. However, taking $\omega_0=10^{-4}rad.s^{-1}$ (instead of $10^{-5}rad.s^{-1}$), leads to the identification of a second-order controller giving an oscillatory behaviour in closed-loop. The consequence is a significant overshoot, which is not acceptable in this application. Furthermore, the command signal $q_s$ rises to $80m^3/s$ when applying a step on the corresponding closed-loop.

\par \leavevmode \par 
In this application, the LDDC method is appealing since it does not require to simulate the complex system described by an irrational transfer function to obtain time-domain data. Only samples of the frequency response of the plant are needed, which can be estimated directly from the irrational transfer function. Moreover, one should notice that controlling such an infinite order model is also quite challenging even for model-based methods. A interesting perspective would be to try this controller on the EDF simulator instead of using the approximate model to validate the performances.


==> tikz/ideal_K.tex <==
\tikzstyle{abstract}=[rectangle, draw=black, rounded corners, fill=blue!5, text centered, anchor=north, text=black, text width=3.5cm]
\tikzstyle{abstract2}=[rectangle, text centered, anchor=north, text=black]
\tikzstyle{block}=[rectangle, draw=black, text centered]
\tikzstyle{comment}=[rectangle, draw=black, rounded corners, fill=red!5, text centered, anchor=north, text=black, text width=3cm]
\tikzstyle{myarrow}=[->, >=open triangle 90, thick]
\tikzstyle{line}=[-, thick]
\tikzstyle{sum}=[draw,circle,text width = 0.3cm]

\begin{tikzpicture}
	\draw
	
	node at (0,0)[]{}
	node [name=ref] {} 
	node at (1,0)[sum](comp){}
	node at (2.2,0)[block](cor){$K^\star$}
	node at (3.7,0)[block](plant){P}
	node at (5.2,0)[](y1){};

	\draw (comp.135) -- (comp.315);
    \draw (comp.225) -- (comp.45);
    \node (plus) [below] at (comp.180) {$+$};
    \node (minus) [below] at (comp.350) {$-$};
	
	\draw[->](ref) -- node[below]{}(comp);
	\draw[->](comp) -- node[above]{}(cor) -- node[above]{}(plant) --node[above]{}(y1);
	\draw[->](4.5,0) -- (4.5,-1) -| node[below]{}(comp);
	\draw[-, dash pattern=on 2pt off 1pt, line width=0.5mm, blue!50] (0.35,-1.2) -- (0.35,0.5) -- (4.7,0.5)--(4.7,-1.2)--node[below]{Reference model $\color{blue!50}{M}$}(0.35,-1.2);
	\end{tikzpicture}

==> tikz/model_ref_pb.tex <==
\tikzstyle{abstract}=[rectangle, draw=black, rounded corners, fill=blue!5, text centered, anchor=north, text=black, text width=3.5cm]
\tikzstyle{abstract2}=[rectangle, text centered, anchor=north, text=black]
\tikzstyle{block}=[rectangle, draw=black, text centered]
\tikzstyle{comment}=[rectangle, draw=black, rounded corners, fill=red!5, text centered, anchor=north, text=black, text width=3cm]
\tikzstyle{myarrow}=[->, >=open triangle 90, thick]
\tikzstyle{line}=[-, thick]
\tikzstyle{sum}=[draw,circle,text width = 0.3cm]

\begin{tikzpicture}
	\draw
	
	node at (0,0)[]{}
	node [name=ref] {} 
	
	node at (-0.5,0)[](r1){}
	node at (2,0.9)[block, fill=blue!10](M){M}
	node at (2,1)[](y){}
	
	node at (1,0)[sum](comp){}
	node at (2,0)[block, fill=red!10](cor){K}
	node at (3,0)[block](plant){P}
	node at (4,0)[](y1){}
	
	node at (4.5,0)[sum](comp2){};
	
	\draw (comp.135) -- (comp.315);
    \draw (comp.225) -- (comp.45);
    \node (plus) [below] at (comp.180) {$+$};
    \node (minus) [below] at (comp.350) {$-$};
    
    \draw (comp2.135) -- (comp2.315);
    \draw (comp2.225) -- (comp2.45);
    \node (plus) [below] at (comp2.180) {$-$};
    \node (minus) [above] at (comp2.50) {$+$};
	
	\draw[->](r1) -- node[]{}(comp);
	\draw[->]node[above]{}(-0.1,0) |- (M) -| node[below]{}(comp2);
	\draw[->](comp) -- node[above]{}(cor) -- node[above]{} (plant) -- node[above]{}(comp2);
	\draw[->](3.5,0) |- (1,-1) -- node[right]{}(comp);
	\draw[-, dash pattern=on 2pt off 1pt, line width=0.5mm, blue!50] (0.2,-1.2) -- (0.2,0.5) -- (4,0.5)--(4,-1.2) -- (0.2,-1.2);
	\draw[->](comp2) -- node[above]{$\varepsilon$}(5.5,0);

	\end{tikzpicture}
